Learning the kernel matrix via predictive low-rank approximations

Efficient and accurate low-rank approximations of multiple data sources are essential in the era of big data. The scaling of kernel-based learning algorithms to large datasets is limited by the O(n^2) computation and storage complexity of the full kernel matrix, which is required by most of the recent kernel learning algorithms. We present the Mklaren algorithm to approximate multiple kernel matrices learn a regression model, which is entirely based on geometrical concepts. The algorithm does not require access to full kernel matrices yet it accounts for the correlations between all kernels. It uses Incomplete Cholesky decomposition, where pivot selection is based on least-angle regression in the combined, low-dimensional feature space. The algorithm has linear complexity in the number of data points and kernels. When explicit feature space induced by the kernel can be constructed, a mapping from the dual to the primal Ridge regression weights is used for model interpretation. The Mklaren algorithm was tested on eight standard regression datasets. It outperforms contemporary kernel matrix approximation approaches when learning with multiple kernels. It identifies relevant kernels, achieving highest explained variance than other multiple kernel learning methods for the same number of iterations. Test accuracy, equivalent to the one using full kernel matrices, was achieved with at significantly lower approximation ranks. A difference in run times of two orders of magnitude was observed when either the number of samples or kernels exceeds 3000.

==> material/align_qr_algorithm.tex <==

\subsection{Efficient learning of optimal kernel weights}
\label{ss:eff_kernel_weigts}

In order to evaluate Eq.~\ref{e:cent_align} and  the parameters $\mx{M}, \mx{a}$ of the optimization problem in Eq.~\ref{e:alignf}, explicit evaluation of each $\mxapps{K}{p} = \mx{G}_p\mx{G}_p$ shall be avoided. Instead, note that $\mxapps{K}{p} = \sum_{c=1}^{c_p} \mx{G}_p(:,c)\mx{G}_p(:,c)^T$.  The alignment to $\mx{K}_Y$ equals:
\beq
    A(\mxapps{K}{p}, \mx{K}_Y) = 
        \frac
        {   \frop{\mxapps{K}{p}}{\mx{K}_Y}    }
        {   \sqrt{  
                \frop{\mxapps{K}{p}}{\mxapps{K}{p}} 
                \frop{\mx{K}_Y}{\mx{K}_Y}
            }
        }     
        = \frac
        {   
           \sum_{c=1}^{c_p} \dotp{\mx{G}_p(:, c)}{\mx{y}}^2 } 
        {   
            n \sqrt{  
                \sum_{c=1}^{c_p}\sum_{c'=1}^{c_p} \dotp{\mx{G}_p(:, c)}{\mx{G}_p(:, c')}^2 
        }} .
\label{e:fastfro}
\eeq

We have used the fact that the Frobenius product between rank-1 outer product matrices equals $\frop{\mx{a}\mx{a}^T}{\mx{b}\mx{b}^T} = \dotp{\mx{a}}{\mx{b}}^2$. The alignment $A(\mxapps{K}{p}, \mx{K}_Y)$ is computed in $O(nc_p^2)$ time, as desired.


% \subsection{Fast independent alignment (\texttt{align\_gg})}


\begin{algorithm}
\SetKwData{Variables}{variables}

\KwIn{$n$ data objects, kernel functions $k_p(., .)$ for $p \in \{1,..,P\}$, class labels $\mx{y} \in \mathbb{R}^{n}$, trade-off parameter $\lambda$, tolerance $\varepsilon$, maximum rank $K$.}
\BlankLine
\KwData{
QR column counter $k \in \mathbb{N}$, 
Chol. column counters $c_1, ..., c_P \in \mathbb{N}^{P}$, 
QR factors $\bigcue{} \in \mathbb{R}^{n \times PK}, 
\bigare{} \in \mathbb{R}^{PK \times PK}$, 
Chol. factors $\mx{G}_1...\mx{G}_P \in \mathbb{R}^{n \times K}$, 
diagonals $\mx{d}_1...\mx{d}_P \in \mathbb{R}^{n}$, 
QP variables $\mxapp{a} \in \mathbb{R}^{P}, \mxapp{M} \in \mathbb{R}^{P \times P}$.
}
\BlankLine
\KwResult{Chol. factors $\mx{G}_1,...,\mx{G}_P$, QR decomp. $\bigcue{}, \bigare{}$, kernel weights $\mxapp{\mu} \in \mathbb{R}^{P}$}
\BlankLine

$k = 0$; $c_1, ..., c_P$ = 0, 0, ..., 0\;  
\BlankLine
Initialize $\mx{d}_1...\mx{d}_P$ as in Eq.\ref{e:icd}\;

\BlankLine
\While{Stopping criteria subject to $\varepsilon$ not met (Section~\ref{ss:stopping})}{

    Select (kernel, pivot column) pair 
    $(k_p(., .), \mx{g}_p)$ that 
    \\ \hspace{5mm} maximizes the gain $\Delta J$ in Eq.~\ref{e:align_qr_cost2}\ for $\bigcue{}, \mx{g}_p, \mx{q}_p, \mx{r}_p, \lambda$;
   
    Perform one step of Chol. decomposition $\mx{G}_p(:, c_p) \leftarrow \mx{g}_p$ ;

    Perform one step of common QR decomposition $\bigcue{}(:, k) \leftarrow \mx{q}_p$, 
       $\bigare{}(:, k) \leftarrow \mx{r}_p$;

    $k = k + 1$;  
    $c_p = c_p + 1$;
}

\For{$p \in \{1,...,P\}$}{
   Let $\mxapp{a}(p)$ = Eq.~\ref{e:fastfro} for $\mx{G}_p, \mx{y}$.
    
    \For{$q \in \{1,...,P\}$}{
        Let $\mxapp{M}(p, q)$ = Eq.~\ref{e:fastfro} for $\mx{G}_p, \mx{G}_q$.
    }
}

Solve QP in Eq.~\ref{e:alignf} for $\mxapp{\mu}$;

\caption{High-level pseudocode for algorithm \texttt{align\_qr}.}
\label{a:align_qr}
\end{algorithm}



==> material/align_qr_analysis_perturbation.tex <==

\subsection{Stopping criteria} 
\label{ss:stopping}

Each kernel $\mx{K}_p$ is approximated by the Cholesky factors $\mx{G}_p$ at each step of Algorithm~\ref{a:align_qr}. A possible stopping criterion is each $\mx{G}_p$ reaching maximum rank $K$ or each approximation $\|\mx{K}_p - \mxapps{K}{p} \|_1$ being within defined tolerance. Alternatively, we outline a stopping criterion based on error guarantees on kernel weights $\mx{\mu}$.

Let $\mx{K}_p, \mx{M}, \mx{a}, \mx{\mu}$ be the original kernel matrix, the parameters and the solution to the optimization problem in Eq.~\ref{e:alignf} without approximations. Let $\mxapps{K}{p}, \mxapp{M}, \mxapp{a},\mxapp{\mu}$ be their approximated counterparts when $\mxapps{K}{p} = \mx{G}_p\mx{G}_p^T$. Associate each $\mx{K}_p$ to the error matrix $\mx{\Xi} = \mx{K}_p - \mxapps{K}{p}$ and let $\ximax = \text{max}_p(\|\mx{\Xi}_p\|_{\infty})$, the maximum residual error. This value is known at each step of Algorithm~\ref{a:align_qr} and is stored in $\text{max}_p(\|\mx{d}_p\|_{\infty})$ by construction of the Cholesky decomposition. Define $R = \text{max}_p(\|\mx{K}_p\|_{\infty})$, the maximum value of base kernels.

Observe that the solution to Eq.~\ref{e:alignf}, $\mx{\mu} = \frac{\mx{M}^{-1}\mx{a}}{\|\mx{M}^{-1}\mx{a}\|_2}$ is equal up to normalization to the solution of the linear system $\mx{M}\mx{\mu} = \mx{a}$. Define perturbations $\mx{\Delta M} = \mx{M} - \mxapp{M}$ and $\mx{\Delta a} = \mx{a} -\mxapp{a}$. Bounding $\| \mx{\Delta M} \|_2, \| \mx{\Delta a} \|_2$ in terms of $\ximax$ would provide error guarantees on the perturbation $\|\mx{\mu} -\mxapp{\mu}\|_2$. 
\vspace{3mm}

\noindent \textbf{Theorem} Given the conditions stated above, the perturbation to the solution linear system $\mx{M}\mx{\mu} = \mx{a}$ is bounded above by   $ \|\mx{\mu} - \mxapp{\mu}\|_2 \leq \frac{2 \delta}{1-r}$ where $\delta$ depends only on the variables  $\ximax, \mxapp{M}, \mxapp{a}$ and $r = \delta \|\mxapp{M}\|_2\|\mxapp{M}^{-1}\|_2 < 1$. 

\noindent \textbf{Proof} Each entry $\mx{\Delta M}_{pq}$ is bounded:
\beq
\begin{split}
\mx{\Delta M}_{pq} &=
    \frop{\mx{K}_p}{\mx{K}_q} - \frop{\mxapps{K}{p}}{\mxapps{K}{q}} =
    \frop{\mx{K}_p}{\mx{K}_q} - \frop{\mx{K}_p - \mx{\Xi}_p }{\mx{K}{q} - \mx{\Xi}_q} = \\\
    &= \frop{\mx{K}_p}{\mx{\Xi}_q} + \frop{\mx{K}_q}{\mx{\Xi}_p} - \frop{\mx{\Xi}_p}{\mx{\Xi}_q}
    \leq \|\mx{K}_p\|_F\|\mx{\Xi}_q\|_F + \|\mx{K}_q\|_F\|\mx{\Xi}_p\|_F  \\
  &\leq n^2(\|\mx{K}_p\|_{\infty}\|\mx{\Xi}_q\|_{\infty} + \|\mx{K}_q\|_{\infty}\|\mx{\Xi}_p\|_{\infty}) \leq 2n^2 R \ximax .
\end{split}
\label{e:boundM}
\eeq

\noindent Here, we have used the distributive property of Frobenius product. The first inequality follows from the Cauchy-Schwartz inequality and the second from the matrix norm relation $\| \mx{A} \|_F \leq n \|\mx{A}\|_2$. The whole perturbation is thus bounded  $\|\mx{\Delta M}\|_2 \leq 2\sqrt{P}n^2R \ximax = B$. The perturbation bound on $\|\mx{\Delta a}\|_2$ is found using a similar argument to give $\|\mx{\Delta a}\|_2 \leq n\sqrt{Pn}\ximax = b$. Choosing  $\delta = \text{max}(B / \|\mxapp{M}\|_2, b/\|\mxapp{a}\|_2)$ yields the theorem. \hfill $\blacksquare$

The bound in the perturbation given by the theorem depends only on the variables  $\ximax, \mxapp{M}, \mxapp{a}$, which are available at each step of Algorithm~\ref{a:align_qr}. The algorithm stops when desired tolerance of the solution $\mx{\mu}$ is achieved.



==> material/align_qr_experiments.tex <==

\section{Experiments}


We evaluate contemporary MKL and predictive low-rank kernel approximation with different datasets. In all experiments, we generate multiple kernel matrices and derive the optimal kernel weights. We evaluate the following methods: kernel weights in proportion to individual alignment \texttt{align}~\cite{Cortes2012}, linear combination of kernel weights with full $\mx{K}_p$  \texttt{alignf}~\cite{Cortes2012}, independent approximation of each $\mx{K}_p$ with CSI \texttt{align\_csi}~\cite{Bach2005} and the proposed method \texttt{align\_qr}.  The resulting kernels are used with the SVM classifier. Only the training samples are used to learn the kernel weights in \texttt{align}, \texttt{alignf} and are allowed to be chosen as pivots in \texttt{align\_csi}, \texttt{align\_qr}. 

The methods are compared on the well-known \texttt{ionosphere}\footnote{\url{https://archive.ics.uci.edu/ml/datasets/Ionosphere}} dataset using the linear kernel $\mx{K}_0$, polynomial kernels (p=2) $\mx{K}_1$, (p=3) $\mx{K}_2$, and Gaussian kernel $\mx{K}_3$.  The Area under the ROC curve (AUC) is reported in Fig.~\ref{f:total}, top.  Considering approximations of all kernels and the obtained predictive subspace, we improve the overall predictive accuracy on the \texttt{ionosphere} dataset with \texttt{align\_qr}. All methods but \texttt{align} identify the most informative kernel (Gaussian). 

The methods are evaluated on a protein-RNA interactions, consisting of 31 experiments relating RNA binding proteins (RBPs) and the target sites on the genome, measured by CLIP-based protocols. We include experiments on 19 proteins\footnote{Proteins used: Ago/EIF2C1-4, Ago2-MNase, Ago2, eIF4AIII, ELAVL1, ELAVL1-MNase, ELAVL1A, ESWR1, FUS, IGF2BP1-3, hnRNPC, hnRNPL, hnRNPL-like, MOV10, PUM2, Nsun2, QKI, TAF15, TIA/TIAL1, U2AF2.} and their technical replicas (in total 31 datasets) from Dorina~\cite{Anders2012} and iCount~\cite{curkcomprehensive}. For each RBP, we sample 500 positive binding sites and 500 random sites from protein coding genes. Each binding site is described with the RNA sequence in the interval $[-50, 50]$ nucleotides within the reported target nucleotide. Five biological sequence kernels (see~\cite{sonnenburg2005large}) are used: linear kernel on sequence 4-mers (\texttt{LIN.}), spectrum kernel (\texttt{SPEC.}),  spectrum with 2 mismatches (\texttt{SPEC. M.}), weighted degree (\texttt{WD}), WD with positional invariance (\texttt{WD P.I.}). 

To evaluate the benefit of joint consideration of the predictive subpsace spanned by pivot columns, we compared the methods \texttt{align\_csi} and \texttt{align\_qr}. Due to space constraints, the average AUC for all 31 proteins in the dataset is reported. The average AUC increases for \texttt{align\_qr} over \texttt{align\_csi} for lower settings of $K$ for the majority of proteins (Fig.~\ref{f:total}, bottom). For the lowest ranks ($K = 2, 3,...$), AUC improves for between 19-23 proteins. Surprisingly, the kernel weights differ significantly between the methods. All methods but \texttt{align} identify \texttt{WD.P.I.} as most informative, which agrees with the fact that CLIP-based protocols identify target nucleotides with a positional variance. 


\begin{figure}[t!]
\centering 
\begin{tabular}{|l|ll|llll|} 
\hline 
Method & Alignment & AUC &  $K_0$&$K_1$&$K_2$&$K_3$ \\ 
\hline
\texttt{align} & 0.163 & 0.804 & 5e-3 & 7e-2 & 9e-1 & 4e-4 \\
\texttt{alignf} & \textbf{0.218} & 0.9  & 4e-3 & 1e-3 & -9e-5 & 1.0 \\
\texttt{align\_csi} & 0.218 & 0.937 &  4e-3 & 1e-3 & -9e-5 & 1.0 \\
\texttt{align\_qr} & 0.203 & \textbf{0.953}  & 5e-3 & -1e-3 & 1e-04 & 1.0 \\
\hline
\end{tabular}


\centering
\raisebox{0.0635\height}{
% \includegraphics[scale=0.9]{img/figure-max-rank-total--6069095968007887793.png}
}
% \includegraphics[scale=0.9]{img/figure-weights-total.png}

\caption{\textbf{Top}: Classification with SVM on the \texttt{ionosphere} dataset. \textbf{Bottom}: Protein-RNA interactions; \texttt{align} (blue), \texttt{alignf} (cyan), \texttt{align\_csi} (yellow), \texttt{align\_qr} (green). \textbf{Left:}  AUC depending on rank $K$ of each $\mx{G}_p$. Black line (right scale) is the number of proteins where \texttt{align\_qr} outperforms \texttt{align\_csi}. \textbf{Right: } Weights of $\mx{K}_p$. 
%\textbf{Right:} the number of selected pivots for each $\mx{K}_p$ by \texttt{align\_qr}.
}
\label{f:total}
\end{figure}




==> material/align_qr_overview.tex <==

\section{Learning the kernel via low-rank approximations}
Assume we are given a data set of arbitrary objects $\mathcal{X} = \{x_1, ..., x_n\}$, target labels $\mx{y} \in \mathbb{R}^{n \times 1}$ and multiple kernel functions $k_1(., .), ..., k_P(., .)$. We propose a joint treatment of i) learning low-rank approximation of the kernel matrices and ii) learning the weights for optimally aligned linear combination. A high-level overview of the proposed method named \texttt{align\_qr} is outlined in Algorithm~\ref{a:align_qr}. 
% In the following, we give detailed description of the main algorithm steps.


\subsection{Learning the approximations with a predictive subspace}
\label{ss:lin_comb_predictive}
Approximations to kernel matrices are learned via Incomplete Cholesky decomposition, which assumes selection of pivots corresponding to training examples at each step until an error tolerance criterion is met. Each kernel matrix $\mx{K}_p$ is approximated by a Cholesky factor $\mx{G}_p$ with $c_p$ columns and the total number of columns is $C = \sum_{p=1}^{P} c_p$. Consider the matrix $\biggee{k-1} = [ \mx{G}_{1}, ..., \mx{G}_{P} ]\in \mathbb{R}^{n \times C} $  with stacked Cholesky factors $\mx{G}_{p}$ in current step $k-1$. On the next step $k$, a new pivot column $\mx{g}_{p}$ is added to $\mx{G}_p \leftarrow [\mx{G}_p, \mx{g}_p] \in \mathbb{R}^{n \times (c_p+1)}$, selected to minimize the cost function when added to the current $\biggee{k} \leftarrow [\biggee{k-1}, \mx{g}_{p}] \in \mathbb{R}^{n \times (C+1)}$:

\beq
\begin{split}
 J(\mx{G_p}, \biggee{k})
 & =  \sum_{p=1}^P \| \mx{K}_p - \mx{G}_{p} \mx{G}_{p}^T \|_1  + \lambda\ \text{min}_{\beta \in \mathbb{R}^{n \times 1}} \| \mx{y} - \mx{\beta}\mx{\biggee{k}} \|_F^2 \\
 & =   \sum_{p=1}^P \| \mx{K}_p - \mx{G}_p\mx{G}_p^T \|_1  + \lambda\ \text{tr} (\mx{y}^T \mx{y} - \mx{y}^T \biggee{k} (\biggee{k}^{T} \biggee{k})^{-1} \biggee{k}^T \mx{y}) \\
\end{split}
\label{e:align_qr_cost1}
\eeq

\noindent The left-hand term is the residual error for each $\mx{K}_p$. The right-hand term is the gain in the range of predictive subspace, resulting from the addition of pivot column $\mx{g}_p$ to the subspace spanned by $\biggee{k}$. This is different than approximating each $\mx{K}_p$, as the correlations among $\mx{K}_p$ are captured via $\biggee{k}$. The weights $\mx{\beta}$ are minimized out by $\mx{\beta} = (\biggee{k}^T\biggee{k})^{-1}\biggee{k}^T\mx{y}$ at the minimal value of Eq.~\ref{e:align_qr_cost1}.

Instead of evaluating Eq.~\ref{e:alignf} at each step, we evaluate the alignment of the subspace spanned by $\biggee{k+1}$ to $\mx{y}$. This is achieved via the QR decomposition, computed in parallel for each $\mx{g}_p$.
% Instead of computing the QR decomposition for each $\mx{G}_p$ separately, 
We keep track of the \emph{complete subspace} spanned by $\biggee{k}$ via the decomposition $\biggee{k} = \bigcue{k}\bigare{k}$, $\bigcue{k} \in \mathbb{R}^{n \times (C+1)}$, $\bigare{k} \in \mathbb{R}^{(C+1) \times (C+1)}$. Rewriting Eq.~\ref{e:align_qr_cost1} by exposing the dependence in $\mx{g}_p$ yields:

\beq
\begin{split}
 J(\mx{g}_p)
 & =   \| \mx{K}_p - \mx{G}_p\mx{G}_p^T \|_1  + \lambda\  \text{tr} (\mx{y}^T\mx{y} - \mx{y}^T\bigcue{k}\bigcue{k}^T\mx{y}) = J_K + \lambda J_Y
\end{split}
\label{e:align_qr_cost2}
\eeq

\noindent The gain in cost defined by Eq.~\ref{e:align_qr_cost2} is evaluated by $\Delta J = \Delta J_K + \lambda \Delta J_Y $, where $\Delta J_K = \| \mx{g}_p\|_2^2$ and $\Delta J_Y = \|\mx{y}^T \mx{q}_p\|_2^2$, where $\mx{q}_p$, $\mx{r}_p$ is the QR decomposition corresponding to $\mx{g}_p$ with respect to $\bigcue{k}$ \footnote{Recomputation of Cholesky and QR decompositions for all remaining indices at each step would yield computational complexity that is above quadratic in $n$. Details of efficient implementation are omitted and the reader is referred to~\cite{Bach2005}.}.


==> material/kernel_choleksy_with_sideinfo.tex <==

\section{Predictive low-rank kernel approximation}
For any symmetric positive definite matrix $\mx{K} \in \mathbb{R}^{n \times n}$ a lower triangular matrix $\mx{G}^T$ can be found such that $\mx{K} = \mx{G}\mx{G}^T$. 
Fine \& Scheinberg~\cite{Fine2001} propose the Incomplete Cholesky decomposition (ICD), approximating \mx{K} with low-rank Cholesky factors $\mx{G} \in \mathbb{R}^{n \times k}$. A vector $\mx{d} \in \mathbb{R}^{n}$ is initialized to the diagonal of \mx{K} as $\mx{d}(i) = \mx{K}(i, i)$. In $k$ steps the pivot column minimizing the upper bound residual error stored in $\mx{d}(i_k)$ is chosen. The approximation at pivot index $i_k$ and the remaining indices $J_k$ is computed as follows:

\beq
\begin{split}
    \mx{G}(i_k, k) &= \sqrt{\mx{d}(i_k)} \\
    \mx{G}(J_k, k) &= \frac{1}{\mx{G}(i_k, k)} (\mx{K}(J_k, i_k) - \sum_{j=1}^{k-1}
    \mx{G}(J_k, j)\mx{G}(i_k, j)) \\
    \mx{d}(j) &= \mx{d}(j) - \mx{G}(j, k)^2 \\
\label{e:icd}
\end{split}
\eeq

\noindent The algorithm terminates after the maximum of $\mx{d}$ is below a defined threshold. Importantly, the evaluation of the full kernel matrix is never required and the computational complexity is $O(nk^2)$. 

Bach \& Jordan~\cite{Bach2005} propose the objective function consisting of two terms: the \emph{approximation error} of \mx{K} and  the \emph{loss} of predicting the target variables $\mx{Y} \in\mathbb{R}^{n \times d}$ in the range space ran($\mx{G}\mx{G}^T)$. The approximation error term is efficiently minimized with the ICD. To minimize the loss term, observe that ran($\mx{G}\mx{G}^T$) is equal to ran(\mx{G}). In order to predict \mx{Y}, it suffices to find a linear combination \mx{\beta} on columns of \mx{G}, yielding the objective with $\lambda$, $\mu$ tradeoff parameters:
\beq
    J(\mx{G}) = \lambda \| \mx{K} - \mx{G}\mx{G}^T \|_1 + \mu\ \text{min}_{\mx{\beta} \in \mathbb{R}^{m \times d}} \| \mx{Y} - \mx{G}\mx{\beta}\|_F^2
\label{e:bach_cost1}
\eeq
Minimizing the right-hand term with respect to \mx{\beta} yields a closed form solution. Pivots $i_k$ in Eq.~\ref{e:icd} are chosen to maximize the gain on the objective in Eq. ~\ref{e:bach_cost1}, efficiently computed via the QR decomposition
    \mx{G} = \mx{Q}\mx{R}, with orthonormal \mx{Q} and upper triangular \mx{R} (see~\cite{golub2012matrix} for details). The iterations of QR decomposition are computed in parallel with ICD, as ran($\mx{G}$) = ran($\mx{Q}$). The optimal pivot is selected by considering the approximation error and alignment of ran($\mx{Q}$) to $\mx{Y}$.



==> material/kernel_mkl_alignment.tex <==

\section{Learning the kernel matrix by alignment optimization}
Instead of using cross-validation to determine the best performing kernel, MKL algorithms optimize the weights $\mx{\mu}_p$ for $P$ different \emph{base kernels} $\mx{K}_p$ to learn the \emph{combined kernel} 
$\mx{K}_{\mu} = \sum_{p=1}^{P} \mx{\mu}_p \mx{K}_p$.
G\"{o}nen\cite{Gonen2011} categorizes MKL approaches based on the learning method, functional form, target function or base learners. 

Shawe-Taylor et al.~\cite{Elisseeff} measure the similarity between a
kernel matrix \mx{K} and the ideal kernel $\mx{K}_Y = \mx{y}\mx{y}^T$ spanned by the labels $\mx{y}$ as the cosine similarity 
$A(\mx{K}, \mx{K}_Y) = \kalign{\mx{K}}{\mx{K}_Y}$, where the Frobenius product $\frop{\mx{K}}{\mx{K}_Y} = \sum_{ij}\mx{K}_{ij}\mx{K}_{Yij}$. 
Cortes et al.~\cite{cortes2010two} extend the notion to the normalized feature space induced by \mx{K}. The \emph{centered kernel} $\mx{K}_c$ and the corresponding \emph{centered alignment} $A_c$ are defined as:
\beq
%    \begin{split}
%                 \mx{K}_c &= (\mx{I} - \frac{\mx{1}\mx{1}^T}{m})\mx{K}(\mx{I} - \frac{\mx{1}\mx{1}^T}{m}) \\
%                 A_c(\mx{K}, \mx{K}_Y) &= \kalign{\mx{K}_c}{\mx{K}_Y} 
%    \end{split}
                 \mx{K}_c = (\mx{I} - \frac{\mx{1}\mx{1}^T}{m})\mx{K}(\mx{I} - \frac{\mx{1}\mx{1}^T}{m}) \ \text{and} \ 
                 A_c(\mx{K}, \mx{K}_Y) = \kalign{\mx{K}_c}{\mx{K}_Y} 
\label{e:cent_align}
\eeq 
where \mx{I} is the indentity matrix and \mx{1} is vector of ones. This generalization has been emprirically shown to be more adequate to inbalanced datasets.

An advantage of kernel alignment is the simplification of MKL algorithms. Cortes et. al \cite{Cortes2012} implement algorithms based on centered alignment; 
\texttt{align} assigns the weights $\mx{\mu}_p$ proportional to the alignment of each centered  $\mx{K}_{k_c}$ with $\mx{K}_Y$. The algorithm \texttt{align} is extended in \texttt{alignf} to optimize over linear combinations of $\mx{\mu}_p$, considering correlations between kernels. 
Let vector
${\mx{a} = (\frop{\mx{K}_{1_c}}{\mx{K}_Y},  ..., \frop{\mx{K}_{p_c}}{\mx{K}_Y})}$ 
and matrix 
$\mx{M}_{ij} = \frop{\mx{K}_{i_c}}{\mx{K}_{j_c}}$. The optimization problem
\beq   
    \text{max}_{\mx{u} \in \mathcal{M}} \kalign{\mx{K}_{\mu_c}}{\mx{K}_Y}
    \label{e:alignf}
\eeq
subject to 
$\mathcal{M} = {\mx{\mu}: \|\mx{\mu}\|_2 = 1}$ 
is a simple QP with a closed form solution 
${\mx{\mu} = \frac{\mx{M}^{-1}\mx{a}}{\|\mx{M}^{-1}\mx{a}\|_2}}$. 
Note since $\frop{.}{.}$ satisfies the properties of a dot product, \mx{M} is positive definite and thus invertible. 
% The results are extended to maximization of the alignment over convex combinations of 
% $\mx{\mu}_p$ and a one-step learning algorithm. 
While the solution of Eq.~\ref{e:alignf} is globally optimal, it assumes the full kernel matrices $\mx{K}_p$. By efficiently calculating $\frop{.}{.}$ from low-rank approximations for $\mx{K}_{k_c}$, we enable solving 
% Eq.~\ref{e:align} and
Eq.~\ref{e:alignf} for large datasets.


==> material/overview.tex <==
% Short overview of the method


\clearpage
\section{Overview}
\subsection{Preliminaries}

The following describes some key issues with predictive Cholesky decomposition, 
mimicking the \emph{Least-angle regression} algorithm. The input is a set of kernels 
\beq
    \{k_1(x, y), k_2(x, y), ... k_p(x,y)\}
\eeq
or a set of  kernel matrices
\beq
    \{ \mx{K}_1, \mx{K}_2, ..., \mx{K}_p \}
\eeq

The approach is described as decomposition of one kernel matrix for brevity, but extends naturally to multiple kernels.


\subsection{Least-angle regression}

Traditional LAR algorithm pseudocode. 

\label{s:lar}

\begin{enumerate}

\item Start with the residual $\mx{r} = \mx{y} - \bar{\mx{y}}$, and regression coefficients $\beta_0, \beta_1, ... \beta_k = 0$.

\item Find the covariate $\mx{x}_j$ most correlated with $\mx{r}$.

\item Move $\beta_j$ towards its least-squares coefficient until another
$\mx{x}_i$ has as much correlation with $\mx{r}$.

\item Move $\beta_j$ and $\beta_i$ in the direction of their \emph{bisector \mx{u}}, 
until some new covariate $\mx{x}_l$ has as much correlation with $\mx{r}$. 
Calculate new bisector. 

\item Repeat until all covariates have been entered, reaching the least-sq.
solution.

\end{enumerate}

The residual error decreases at every step, because access to all covariates is assumed. For our method, covriates are added "on the fly". We require random ordering of columns: 

\begin{enumerate}
\item Start with the residual $\mx{r} = \mx{y} - \bar{\mx{y}}$, and regression
coefficients $\beta_0, \beta_1, ... \beta_k = 0$.

\item {\color{blue} Add a random covariate $\mx{x}_j$ to the model $\mx{r}$.}

\item Move $\beta_j$ towards its least-squares coefficient until another
$\mx{x}_i$ has as much correlation with $\mx{r}$.

\item Move $\beta_j$ and $\beta_i$ in the direction of their \emph{bisector \mx{u}}, 
until some new covariate $\mx{x}_l$ has as much correlation with
$\mx{r}$.

\item Repeat until {\color{blue} at most k} covariates have been entered, reaching the least-sq.
solution {\color{blue} for those k covariates}.

\end{enumerate}


\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{overview_lar.png}
    \caption{First step of the classic LAR algorithm.}
    \label{f:LAR}
\end{figure}


\clearpage
\subsection{Computation of quantities required for LAR in the Cholesky decomposition.}
\label{s:icd_lookahead}
In the Cholesky decomposition, covariates $\mx{x}_i$ are individual pivot columns $\mx{g}_i$. 
At each step of the cholesky decomposition, we have:
\begin{itemize}
    \item Cholesky factors $\mx{G}_k$.
    \item Look-ahead Cholesky factors $\mx{G}_{k+\delta}$-
\end{itemize}

LAR algorithm assumes the following quantities for each covariate:
\begin{itemize}
   \item correlation with bisector $\mx{g}_i^T\mx{u}/\|\mx{g}_i\|$,
   \item correlation with residual $\mx{g}_i^T\mx{r}/\|\mx{g}_i\|$,
\end{itemize}

By definition of Cholesky decomposition, a new column $\mx{g}_i$ at step $k$ is defined. Constants $C$ cancel out in both the above expressions.
\beq
   \mx{g}_i = (K(:,i) - \mx{G}_{k-1}\mx{G}_{k-1}^T(:, i)) \times C
\eeq

{\color{blue} Key simplification}. Use the look-ahead decomposition to speed-up the computation.
\beq
\begin{split}
   \hat{\mx{g}_i} &= (\mx{G}_{k+\delta}\mx{G}_{k+\delta}^T - \mx{G}_{k-1}\mx{G}_{k-1}^T(:, i)) \times C \\
                  &= (\mx{G}_{k:k+\delta}\mx{G}_{k:k+\delta}^T) \times C
\end{split}
\eeq

This makes the required computations more effiecient ($O(n\delta^2) < O(n^2)$). 
Because the values are approximate, the {\color{blue} true column $\mx{g}_i$ is known only after it is added to the decomposition.}
Also, its true correlation with residual \mx{r} and the bisector \mx{u} are known only then. 
This is the motivation for LAR algorithm with random ordering of added covariates. 
Nevertheless, the least squares solution for the final set of covariates in $\mx{G}_k$ is still found. 

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{overview_lookahead.png}
\caption{Illustration of lookahead $\delta$ parameter.}
\label{f:overview_lookahead}
\end{figure}


\subsection{L2-regularization}
The Ridge regression (L2-norm regularization) is achieved simply by augmenting the data as follows.

\begin{equation*}
\mx{X}^* = (1+\lambda)^{-1/2} \begin{pmatrix}\mx{X} \\ \sqrt{\lambda}\mx{I}\end{pmatrix}
\end{equation*}
\begin{equation*}
\mx{y}^* =
\begin{pmatrix} \mx{y} \\ \mx{0}
\end{pmatrix}.
\end{equation*}

Then, the least-squares solution of $\mx{X}^*, \mx{y}^*$ is equivalent ot Ridge regression of the original data $\mx{X}, \mx{y}$. For proof, see ref.~\cite{Zou2005}.

This augmentation does not imply additional computational costs to the algorithm and it is straghtforward to include the augmentation in computations in Section~\ref{s:lar} and Section~\ref{s:icd_lookahead}.


\clearpage
\subsection{Algorithm overview}

The high level pseudocode for recomnstructing a kernel matrix \mx{K} given the regression targets \mx{y} is as follows.

\begin{enumerate}

\item Compute $\delta$ look-ahead Cholesky factors, $\mx{G}_\delta$.

\item Start with empty bisector $\mx{u} = \mx{0}$, empty regression line $\mx{\mu} = \mx{0}$,  and residual $\mx{r} = \mx{y} - \bar{\mx{y}}$.

At each step $k=1..K$:
\begin{enumerate}

    \item Choose column according correlations in Section~\ref{s:icd_lookahead}. Compute its true
Cholesky factor $\mx{g}$ . Add it to the decomposition (set of covariates)  \\ $\mx{G}_k \leftarrow [ \mx{G}_{k-1}, \mx{g}_k ] $. Modify the look ahead decomposition $\mx{G}_{k+\delta}$. 

    \item Modify bisector \mx{u} and residual \mx{r} such that all covariates in $\mx{G}_k$ are equally correlated to the residual.

    \item Modify regression line until a new variable is {\color{blue} predicted} to be equally correlated to current set of covariates, by choosing appropriate gradient $\gamma$. Use values in Section~\ref{s:icd_lookahead}.
        \beq
            \hat{\mx{\mu}} = \mx{\mu} + \gamma \mx{u}.
        \eeq
    \item Get new residual $\mx{r} = \mx{y} - \hat{\mx{\mu}} - \bar{\mx{y}}$

\end{enumerate}

\item Obtain the regression coeffients \mx{\beta} by least-squares solution $\mx{G}_K \mx{\beta} = \mx{\mu}$. 

\end{enumerate}



\subsection{Prediction}

Any Cholesky decomposition using $k$ pivot columns with indices $ S = {i_1, i_2, ... i_k}$ yields the 
same approximation as the Nystrom decomposition using the same set of indices:
\beq
    \mx{G}_k\mx{G}_k^T = \mx{K}_{:, S}\mx{K}^{-1}_{S, S}\mx{K}_{S, :}
\eeq

Assume a training set of indices $TR$ and test set $TE$. The Cholesky factors for test indices are obtained by simple 
linear algebra as follows:
\beq
   \mx{G}_{TE} = (\mx{G}_{TR}^T\mx{G}_{TR})^{-1} \mx{G}_{TR}^T \mx{K}_{TR, S}\mx{K}^{-1}_{S, S}\mx{K}_{S, TE}
\eeq

The regression coefficients obtained by the algorithm can thus be used on the Cholesky factors for test indices. 
The linear transform
\beq
(\mx{G}_{TR}^T\mx{G}_{TR})^{-1} \mx{G}_{TR}^T \mx{K}_{TR, S}\mx{K}^{-1}_{S, S}
\eeq
is independent of the test set and can be computed only once.



==> material/supplement_beta_norm_bound.tex <==

\subsection{Bound on $\ell_p$ norm of primal/dual coefficients}

\emph{Proposition}. Let $\mx{\beta}_{G}$ and $\mx{\beta}_{\Phi}$ be the Ridge regression weights in the input spaces associated to matrices \mx{G} and \mx{\Phi}, respectively. Then, the following relation holds
\beq
    \|\mx{\beta}_{\Phi}\|_p \leq \|\mx{\beta}_{G}\|_p \| \mx{G}^{\dagger} \|_p \|\mx{\Phi}\|_p
\eeq

where $\cdot^{\dagger}$ denotes the Moore-Penrose pseudo-inverse, and $\| \cdot \|_p$ denotes any $\ell_p$ norm (used in a vector/matrix sense where appropriate).

\emph{Proof}. Let the Cholesky factor $\mx{G}$ be the input space associated to the regression problem. By assumption of RR, the weights $\mx{\beta}_G$ are given as some combination of the input points, given by the dual coefficients $\mx{\alpha}$:

\beq
\mx{\beta}_{G} = \mx{G}\mx{\alpha} = \mx{G}{\color{red} (\mx{G}\mx{G}^T + \lambda\mx{I})\mx{y}}
\label{e:rr_primal_g}
\eeq

The situation for the input space $\mx{\Phi}$ is analogous:
\beq
\mx{\beta}_{ \Phi } = \Phi\mx{\alpha} = \Phi{\color{red}(\mx{G}\mx{G}^T + \lambda\mx{I})\mx{y}}.
\eeq

In our case, Eq.~\ref{e:rr_primal_g} represents and underdetermined linear system of equations with dual coefficients $\mx{\alpha}$ as unknowns. One way to solve Eq.~\ref{e:rr_primal_g} for $\mx{\alpha}$ is using the pseudo-inverse $\mx{G}^{\dagger}$, yielding the minimal euclidead norm solutions. This solution would yield controllable bounds on the norm $\|\mx{\beta}_\Phi\|_p$ but would in general not be sparse.

Another option is to solve the \emph{mathing basis pursuit} problem, that will give a sparse solution with respect to $\|\mx{\alpha}\|_1$. See \url{http://spams-devel.gforge.inria.fr/} for details. The relation between the norms of primal coefficients are now less clear (however, $\|\mx{\beta}_\Phi\|_p$ would still be influenced by $\|\mx{\beta}_G\|_p$). 


==> material/supplement_greedy_low_rank_kernel.tex <==
% Supplementary material to from the complete article.


\section{Supplementary material}

\subsection{Greedy low-rank approximations to the kernel matrix}

Let $\mx{K} \in \mathbb{R}^{n \times n}$ be any symmetric matrix. In this
section, we present greedy methods for low-rank approximation of form $\mx{K} =
\mx{G}\mx{G}^T$, where $\mx{G} \in \mathbb{R}^{n \times r}$ is a matrix of column
rank $r$. The problem is well known in numerical linear algebra and can be solved in
context of kernel methods with methods such as the Nystr\"om
approximation~\cite{Kumar2012,Williams2001,Li2015}, Random Fourier
Features\cite{Rahimi2007,Rahimi2009,Le2013a,Yang2014}, or direct approximation
of the kernel function~\cite{Vedaldi2012}.


\subsubsection{Incomplete Cholesky Decomposition}

Fine and Shai~\cite{Fine2001} proposed Incomplete Cholesky Decomposition (ICD)
as a modification of the original Cholesky
decomposition~\cite{golub2012matrix}.  The former reconstructs $\mx{K}$ exactly
with time complexity $O(n^3)$. ICD selects pivot columns in \mx{G} using a
greedy strategy and employs the strategy of early stopping after selecting up
to $r$ pivot columns. This results in reduction of time complexity to
$O(nr^2)$.

The algorithm starts by initializing the diagonal vector $\mx{d}(i) = \mx{K}(i,
i)$. These values represent lower bounds on the gain of the approximation error
and are updated after each iteration.  The active set $\mathcal{I}$ holds the
indices of selected pivot columns and the set
$\mathcal{J}$ holds the remaining indices. At iteration $k$, the pivot column
at index $i_k$ is selected and the current approximation is updated according
to the current residual $(\mx{K}(\mathcal{J}, k) - \mx{G}(\mathcal{J}, :)\mx{G}^T(i_k, :))$.

It is worth to note that using suitable row permutations, $\mx{G}$ can be made into
an upper-triangular matrix.  As will become clear later, we choose not to adopt
this strategy.

\begin{algorithmic}
\Function{ICD}{\mx{K}, $r$}
\State $\mx{d} \gets \text{diag(\mx{K})}$
\State $\mathcal{I} \gets \emptyset$, $\mathcal{J} \gets \{1, 2, ..., n\}$
% \State $\mathcal{J} \gets \{1, 2, ..., n\}$
\For {$k = 1 \ .. \  r$}
\State  $i_k \gets \text{argmax}(\mx{d})$
\State  $\mx{G}(i_k, k) \gets \sqrt{\mx{d}(i_k)}$

\State $\mathcal{I} \gets \mathcal{I} \cup \{i\}$, $\mathcal{J} \gets \mathcal{J} \setminus \{i\}$
% \State $\mathcal{J} \gets \mathcal{J} \setminus \{i\}$
\For{$j \notin \mathcal{J}$}
\State  $\mx{G}(j, k) \gets \frac{1}{\mx{G}(i_k, k)} (\mx{K}(j, k) - \mx{G}(j, :)\mx{G}^T(i_k, :))$
\State $\mx{d}(j) \gets \mx{d}(j) - \mx{G}(j, k)^2$
\EndFor
\EndFor
\EndFunction
\end{algorithmic}



\subsubsection{Cholesky with Side-Information}

Bach \& Jordan~\cite{Bach2005} propose Cholesky with Side-Information (CSI).
The approximation is assumed to be made in the context of supervised learning,
with available training response matrix $\mx{Y} \in\mathbb{R}^{n \times d}$,
i.e., simultaneous regression on $d$ response variables. 

The global objective function is composed of two terms: the \emph{approximation
error} of \mx{K} (ICD) and the \emph{loss} of predicting the target variables
$\mx{Y} \in\mathbb{R}^{n \times d}$ in the range space ran($\mx{G}\mx{G}^T)$. 

\beq J(\mx{G}) = \lambda \| \mx{K} - \mx{G}\mx{G}^T \|_1 + \mu\
\text{min}_{\mx{\beta} \in \mathbb{R}^{m \times d}} \| \mx{Y} -
\mx{G}\mx{\beta}\|_F^2 \label{e:bach_cost1_copy} \eeq

The $\lambda$ and $\mu$ are trade-off parameters. Setting $\mu=0$ yields the
ICD.  Observe that the right-hand term is formulated as an optimization
problem. Minimizing with respect to \mx{\beta} yields a closed form solution.
Pivots $i_k$ in Eq.~\ref{e:icd} are chosen to maximize the gain on the
objective in Eq. ~\ref{e:bach_cost1_copy}. Computing the derivative with respect to
a column $\mx{g}_i$ and maximizing yields the new pivot selection criterion:

\beq \Delta J = \| \mx{g}_i \|^2 + \| \mx{Y}^T\mx{q}_i\|^2,
\label{e:bach_gain2} \eeq where $\mx{q}_i$ is the corresponding column in the
QR decomposition.

We build on the essential contribution of ref.~\cite{Bach2005} which presents a
method to compute Eq.~\ref{e:bach_gain2} efficiently, using look-ahead
decompositions. Briefly, in ICD, the right-hand term of Eq.~\ref{e:bach_gain2},
$\| \mx{g}_i \|^2$ was estimated implicitly by using the lower-bound in
$\mx{d}$. The right-hand term is more complicated; instead of naively
recomputing its value in each iteration, the authors use the following
observation. By definition, we have

\beq \mx{g}_i = \frac{(\mx{K} - \mx{G}_k\mx{G}_k^T)(:, i)}{\sqrt{\mx{d}(i, i)}}
\eeq    

Using a emph{look-ahead} low-rank approximation, $\mx{L} = \mx{G}_{k
+\delta}\mx{G}_{k+\delta}^T$, the unknown column $\mx{g}_i$ is approximated as 

\beq \mxapp{g}_i = \frac{(\mx{L} - \mx{G}_k\mx{G}_k^T)(:, i)}{\sqrt{\mx{d}(i,
i)}} \eeq


Observe that $\mx{L} - \mx{G}_k\mx{G}_k^T =
\mx{G}_{k:k+\delta}\mx{G}_{k:k+\delta}^T.$ 
This makes the required computations more efficient, as will be illustrated more
explicitly in the derivation of our algorithm.

